RSK with a twist, mirabolic Steinberg variety, and Pak--Postnikov representations

There is a beautiful interplay between the classical Robinson--Schensted correspondence and the Steinberg variety, which is the union of conormal components of $Fl(V) \times Fl(V)$. The irreducible components of the Steinberg variety gives the geometric interpretation of RS, and Pak--Postnikov description of RS as U,D operators is the combinatorics shadow of the $S_n\times S_n$-representation inside the top homology of the Steinberg variety. We study the conormal components of $Fl(V) \times Fl(V) \times L(\lambda)$, where $L(\lambda)$ is an irreducible representation of $GL(V)$. We show that there are only three families of $L(\lambda)$ such that $Fl(V)\times Fl(V) \times L(\lambda)$ has finitely many orbits. These families are determinant twists of classical RS, Travkin's mirabolic RSK and its Fourier dual. We extend the combinatorial interpretation of RS in terms of U,D operators to mirabolic RSK. Finally, we give a filtration of the top homology of the mirabolic Steinberg variety in which each graded piece is a Pak--Postnikov $S_n \times S_n$-representations.

==> tikz.tex <==
%%%%%%%%%%% ----- shadow31862547 ----- %%%%%%%


% \def\perm{3,1,8,6,2,5,4,7}

% \foreach \w [count=\i] in \perm {
% \xdef\permsize{\i}
% }

% \draw[step=1, thin]
% (0,0) grid (\permsize,\permsize);

% \draw[blue, very thick] (7.5,8) -- (7.5,1.5) -- (2.5,1.5) -- (2.5,0.5) -- (0,0.5);

% \draw[blue, very thick] (6.5,8) -- (6.5,4.5) -- (5.5,4.5) -- (5.5,3.5) -- (3.5,3.5) -- (3.5,2.5) -- (0,2.5);

% \draw[blue, very thick] (4.5,8) -- (4.5,6.5) -- (0.5,6.5) -- (0.5,5.5) -- (0,5.5);(0,2.5);

% \draw[blue, very thick] (1.5,8) -- (1.5,7.5) -- (0,7.5);

% \foreach \w [count=\i] in \perm {
% \node[fill = white, circle] at ({\i-0.5},{\permsize - \w + 0.5}) {$\times$};
% }




%%%%%%%%%%% ----- RBtoP ----- %%%%%%%

% \draw[step=1, thin] (0,0) grid (5,5);

% \draw[blue, very thick] (4.5,5.5) -- (4.5,4.5) -- (2.5,4.5) -- (2.5,1.5) -- (-0.5,1.5);

% \draw[blue, very thick] (1.5,5.5) -- (1.5,2.5) -- (-0.5,2.5); 

% \node[fill = white, circle] at (0.5,0.5) {$\times$};
% \node[fill = white, circle] at (1.5,2.5) {$\otimes$};
% \node[fill = white, circle] at (2.5,1.5) {$\otimes$};
% \node[fill = white, circle] at (3.5,3.5) {$\times$};
% \node[fill = white, circle] at (4.5,4.5) {$\otimes$};

% \node[fill = white, circle] at (2.5,4.5) {\textcolor{red}{$\times$}};

% \node[fill = white, circle] at (-0.5,1.5) {\textcolor{green}{$\times$}};
% \node[fill = white, circle] at (-0.5,2.5) {\textcolor{green}{$\times$}};
% \node[fill = white, circle] at (1.5,5.5) {\textcolor{green}{$\times$}};
% \node[fill = white, circle] at (4.5,5.5) {\textcolor{green}{$\times$}};







%%%%%%%%%%% ----- gd2341 ----- %%%%%%%


% \begin{tikzcd}[ampersand replacement=\&, sep = small]
%     \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \\
%     \&\&\&\&\&\&\& \times \\
%     \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\&
%     \ctab{\begin{ytableau} {} \end{ytableau}} \\
%     \& \times \\
%     \varnothing \&\&
%     \ctab{\begin{ytableau} {} \end{ytableau}} \&\&
%     \ctab{\begin{ytableau} {} \end{ytableau}} \&\&
%     \ctab{\begin{ytableau} {} \end{ytableau}} \&\&
%     \ctab{\begin{ytableau} {} \\ {} \end{ytableau}} \\
%     \&\&\& \times \\
%     \varnothing \&\&
%     \ctab{\begin{ytableau} {} \end{ytableau}} \&\&
%     \ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\&
%     \ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\&
%     \ctab{\begin{ytableau} {} & {} \\ {} \end{ytableau}} \\
%     \&\&\&\&\& \times \\
%     \varnothing \&\&
%     \ctab{\begin{ytableau} {} \end{ytableau}} \&\&
%     \ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} & {} \\ {} \end{ytableau}}
%     \arrow[no head, from=1-1, to=1-3]
%     \arrow[no head, from=1-1, to=3-1]
%     \arrow[no head, from=1-3, to=1-5]
%     \arrow[no head, from=1-3, to=3-3]
%     \arrow[no head, from=1-5, to=1-7]
%     \arrow[no head, from=1-5, to=3-5]
%     \arrow[no head, from=1-7, to=1-9]
%     \arrow[no head, from=1-7, to=3-7]
%     \arrow[no head, from=1-9, to=3-9]
%     \arrow[no head, from=3-1, to=3-3]
%     \arrow[no head, from=3-1, to=5-1]
%     \arrow[no head, from=3-3, to=3-5]
%     \arrow[no head, from=3-3, to=5-3]
%     \arrow[no head, from=3-5, to=3-7]
%     \arrow[no head, from=3-5, to=5-5]
%     \arrow[no head, from=3-7, to=3-9]
%     \arrow[no head, from=3-7, to=5-7]
%     \arrow[no head, from=3-9, to=5-9]
%     \arrow[no head, from=5-1, to=5-3]
%     \arrow[no head, from=5-1, to=7-1]
%     \arrow[no head, from=5-3, to=5-5]
%     \arrow[no head, from=5-3, to=7-3]
%     \arrow[no head, from=5-5, to=5-7]
%     \arrow[no head, from=5-5, to=7-5]
%     \arrow[no head, from=5-7, to=5-9]
%     \arrow[no head, from=5-7, to=7-7]
%     \arrow[no head, from=5-9, to=7-9]
%     \arrow[no head, from=7-1, to=7-3]
%     \arrow[no head, from=7-1, to=9-1]
%     \arrow[no head, from=7-3, to=7-5]
%     \arrow[no head, from=7-3, to=9-3]
%     \arrow[no head, from=7-5, to=7-7]
%     \arrow[no head, from=7-5, to=9-5]
%     \arrow[no head, from=7-7, to=7-9]
%     \arrow[no head, from=7-7, to=9-7]
%     \arrow[no head, from=7-9, to=9-9]
%     \arrow[no head, from=9-1, to=9-3]
%     \arrow[no head, from=9-3, to=9-5]
%     \arrow[no head, from=9-5, to=9-7]
%     \arrow[no head, from=9-7, to=9-9]
% \end{tikzcd}






%%%%%%%%%%% ----- Xi-pp ----- %%%%%%%

% \begin{tikzcd}[ampersand replacement=\&, sep = small]
%     \&\& \ctab{\begin{ytableau} {} & {} & {} \\ {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \\
% 	\&\&\&\&\& \times \&\&\&\&\&\& \times \\
% 	\ctab{\begin{ytableau} {} & {} & {} \\ {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \&\& \varnothing \\
% 	\&\&\&\&\&\&\& \times \\
% 	\ctab{\begin{ytableau} {} & {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \&\& \varnothing \\
% 	\&\&\&\&\&\&\&\&\& \times \\
% 	\ctab{\begin{ytableau} {} & {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \\
% 	\& \times \\
% 	\ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \\
% 	\& \times \\
% 	\ctab{\begin{ytableau} {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \\
% 	\&\&\& \times \\
% 	\varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing \&\& \varnothing
% 	\arrow[no head, from=1-3, to=1-5]
% 	\arrow[no head, from=1-3, to=3-3]
% 	\arrow[no head, from=1-5, to=1-7]
% 	\arrow[no head, from=1-5, to=3-5]
% 	\arrow[no head, from=1-7, to=1-9]
% 	\arrow[no head, from=1-7, to=3-7]
% 	\arrow[no head, from=1-9, to=1-11]
% 	\arrow[no head, from=1-9, to=3-9]
% 	\arrow[no head, from=1-11, to=1-13]
% 	\arrow[no head, from=1-11, to=3-11]
% 	\arrow[no head, from=1-13, to=3-13]
% 	\arrow[no head, from=3-1, to=3-3]
% 	\arrow[no head, from=3-1, to=5-1]
% 	\arrow[no head, from=3-3, to=3-5]
% 	\arrow[no head, from=3-3, to=5-3]
% 	\arrow[no head, from=3-5, to=3-7]
% 	\arrow[no head, from=3-5, to=5-5]
% 	\arrow[no head, from=3-7, to=3-9]
% 	\arrow[no head, from=3-7, to=5-7]
% 	\arrow[no head, from=3-9, to=3-11]
% 	\arrow[no head, from=3-9, to=5-9]
% 	\arrow[no head, from=3-11, to=3-13]
% 	\arrow[no head, from=3-11, to=5-11]
% 	\arrow[no head, from=3-13, to=5-13]
% 	\arrow[no head, from=5-1, to=5-3]
% 	\arrow[no head, from=5-1, to=7-1]
% 	\arrow[no head, from=5-3, to=5-5]
% 	\arrow[no head, from=5-3, to=7-3]
% 	\arrow[no head, from=5-5, to=5-7]
% 	\arrow[no head, from=5-5, to=7-5]
% 	\arrow[no head, from=5-7, to=5-9]
% 	\arrow[no head, from=5-7, to=7-7]
% 	\arrow[no head, from=5-9, to=5-11]
% 	\arrow[no head, from=5-9, to=7-9]
% 	\arrow[no head, from=5-11, to=5-13]
% 	\arrow[no head, from=5-11, to=7-11]
% 	\arrow[no head, from=5-13, to=7-13]
% 	\arrow[no head, from=7-1, to=7-3]
% 	\arrow[no head, from=7-1, to=9-1]
% 	\arrow[no head, from=7-3, to=7-5]
% 	\arrow[no head, from=7-3, to=9-3]
% 	\arrow[no head, from=7-5, to=7-7]
% 	\arrow[no head, from=7-5, to=9-5]
% 	\arrow[no head, from=7-7, to=7-9]
% 	\arrow[no head, from=7-7, to=9-7]
% 	\arrow[no head, from=7-9, to=7-11]
% 	\arrow[no head, from=7-9, to=9-9]
% 	\arrow[no head, from=7-11, to=7-13]
% 	\arrow[no head, from=7-11, to=9-11]
% 	\arrow[no head, from=7-13, to=9-13]
% 	\arrow[no head, from=9-1, to=9-3]
% 	\arrow[no head, from=9-1, to=11-1]
% 	\arrow[no head, from=9-3, to=9-5]
% 	\arrow[no head, from=9-3, to=11-3]
% 	\arrow[no head, from=9-5, to=9-7]
% 	\arrow[no head, from=9-5, to=11-5]
% 	\arrow[no head, from=9-7, to=9-9]
% 	\arrow[no head, from=9-7, to=11-7]
% 	\arrow[no head, from=9-9, to=9-11]
% 	\arrow[no head, from=9-9, to=11-9]
% 	\arrow[no head, from=9-11, to=9-13]
% 	\arrow[no head, from=9-11, to=11-11]
% 	\arrow[no head, from=9-13, to=11-13]
% 	\arrow[no head, from=11-1, to=11-3]
% 	\arrow[no head, from=11-1, to=13-1]
% 	\arrow[no head, from=11-3, to=11-5]
% 	\arrow[no head, from=11-3, to=13-3]
% 	\arrow[no head, from=11-5, to=11-7]
% 	\arrow[no head, from=11-5, to=13-5]
% 	\arrow[no head, from=11-7, to=11-9]
% 	\arrow[no head, from=11-7, to=13-7]
% 	\arrow[no head, from=11-9, to=11-11]
% 	\arrow[no head, from=11-9, to=13-9]
% 	\arrow[no head, from=11-11, to=11-13]
% 	\arrow[no head, from=11-11, to=13-11]
% 	\arrow[no head, from=11-13, to=13-13]
% 	\arrow[no head, from=13-1, to=13-3]
% 	\arrow[no head, from=13-3, to=13-5]
% 	\arrow[no head, from=13-5, to=13-7]
% 	\arrow[no head, from=13-7, to=13-9]
% 	\arrow[no head, from=13-9, to=13-11]
% 	\arrow[no head, from=13-11, to=13-13]
% \end{tikzcd}









%%%%%%%%%%% ----- 2nGD ----- %%%%%%%


% \begin{tikzcd}[ampersand replacement=\&, sep = small]
%     \ctab{\begin{ytableau} {} & {} & {} \\ {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \\
% 	\&\&\& \times \&\&\&\&\&\& \\
% 	\ctab{\begin{ytableau} {} & {} \\ {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \\
% 	\&\&\&\&\&\&\&\&\& \times \\
% 	\ctab{\begin{ytableau} {} & {} \\ {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} & {} \end{ytableau}} \&\& \ctab{\begin{ytableau} {} \end{ytableau}} \&\& \varnothing \&\& \varnothing
% 	\arrow[no head, from=1-1, to=1-3]
% 	\arrow[no head, from=1-3, to=1-5]
% 	\arrow[no head, from=1-5, to=1-7]
% 	\arrow[no head, from=1-7, to=1-9]
% 	\arrow[no head, from=1-9, to=1-11]
% 	\arrow[no head, from=3-1, to=3-3]
% 	\arrow[no head, from=3-3, to=3-5]
% 	\arrow[no head, from=3-5, to=3-7]
% 	\arrow[no head, from=3-7, to=3-9]
% 	\arrow[no head, from=3-9, to=3-11]
% 	\arrow[no head, from=5-1, to=5-3]
% 	\arrow[no head, from=5-3, to=5-5]
% 	\arrow[no head, from=5-5, to=5-7]
% 	\arrow[no head, from=5-7, to=5-9]
% 	\arrow[no head, from=5-9, to=5-11]
% 	\arrow[no head, from=1-1, to=3-1]
% 	\arrow[no head, from=1-3, to=3-3]
% 	\arrow[no head, from=1-5, to=3-5]
% 	\arrow[no head, from=1-7, to=3-7]
% 	\arrow[no head, from=1-9, to=3-9]
% 	\arrow[no head, from=1-11, to=3-11]
% 	\arrow[no head, from=3-1, to=5-1]
% 	\arrow[no head, from=3-3, to=5-3]
% 	\arrow[no head, from=3-5, to=5-5]
% 	\arrow[no head, from=3-7, to=5-7]
% 	\arrow[no head, from=3-9, to=5-9]
% 	\arrow[no head, from=3-11, to=5-11]
% \end{tikzcd}
